Uncertainty Estimation in Autoregressive Structured Prediction

Uncertainty estimation is important for ensuring safety and robustness of AI systems. While most research in the area has focused on un-structured prediction tasks, limited work has investigated general uncertainty estimation approaches for structured prediction. Thus, this work aims to investigate uncertainty estimation for autoregressive structured prediction tasks within a single unified and interpretable probabilistic ensemble-based framework. We consider: uncertainty estimation for sequence data at the token-level and complete sequence-level; interpretations for, and applications of, various measures of uncertainty; and discuss both the theoretical and practical challenges associated with obtaining them. This work also provides baselines for token-level and sequence-level error detection, and sequence-level out-of-domain input detection on the WMT'14 English-French and WMT'17 English-German translation and LibriSpeech speech recognition datasets.

==> BDL_poster/abbreviations.tex <==
% Abbreviations

\newcommand{\iid}{independent and identically distributed\xspace}

\newcommand{\logl}{log-likelihood\xspace}
\newcommand{\Logl}{Log-likelihood\xspace}
\newcommand{\LL}{\textsc{ll}\xspace}
\newcommand{\logls}{{\logl}s\xspace}
\newcommand{\Logls}{{\Logl}s\xspace}
\newcommand{\LLs}{{\LL}s\xspace}

\newcommand{\mlh}{maximum likelihood\xspace}
\newcommand{\Mlh}{Maximum likelihood\xspace}
\newcommand{\ML}{\textsc{ml}\xspace}

\newcommand{\mle}{maximum-likelihood estimation\xspace}
\newcommand{\Mle}{Maximum-likelihood estimation\xspace}
\newcommand{\MLE}{\textsc{mle}\xspace}
\newcommand{\mlee}{maximum-likelihood estimate\xspace}
\newcommand{\mled}{maximum-likelihood estimated\xspace}
\newcommand{\mles}{maximum-likelihood estimates\xspace}

\newcommand{\map}{maximum \emph{a posteriori}\xspace}
\newcommand{\Map}{Maximum \emph{a posteriori}\xspace}
\newcommand{\MAP}{\textsc{map}\xspace}

\newcommand{\cml}{conditional maximum likelihood\xspace}
\newcommand{\Cml}{Conditional maximum likelihood\xspace}
\newcommand{\CML}{\textsc{cml}\xspace}

\newcommand{\mbr}{minimum Bayes risk\xspace}
\newcommand{\Mbr}{Minimum Bayes risk\xspace}
\newcommand{\MBR}{\textsc{mbr}\xspace}

\newcommand{\mpe}{minimum phone error\xspace}
\newcommand{\Mpe}{Minimum phone error\xspace}
\newcommand{\MPE}{\textsc{mpe}\xspace}

\newcommand{\expm}{expect\-ation--maxi\-misation\xspace}
\newcommand{\Expm}{Expect\-ation--maxi\-misation\xspace}
\newcommand{\EM}{\textsc{em}\xspace}

\newcommand{\kl}{Kullback-Leibler\xspace}
\newcommand{\Kl}{\kl}
\newcommand{\KL}{\textsc{kl}\xspace}

% Techniques

\newcommand{\mllr}{maximum-likelihood linear regression\xspace}
\newcommand{\Mllr}{Maximum-likelihood linear regression\xspace}
\newcommand{\MLLR}{\textsc{mllr}\xspace}
\hyphenation{mllr}

\newcommand{\fe}{front-end}
\newcommand{\Fe}{Front-end}
\newcommand{\FE}{\textsc{fe}}

\newcommand{\cmllr}{constrained \mllr}
\newcommand{\Cmllr}{Constrained \mllr}
\newcommand{\CMLLR}{\textsc{cmllr}\xspace}
\hyphenation{cmllr}

\newcommand{\lda}{linear discriminant analysis\xspace}
\newcommand{\Lda}{Linear discriminant analysis\xspace}
\newcommand{\LDA}{\textsc{lda}\xspace}

\newcommand{\hda}{heteroscedastic discriminant analysis\xspace}
\newcommand{\Hda}{Heteroscedastic discriminant analysis\xspace}
\newcommand{\HDA}{\textsc{hda}\xspace}

\newcommand{\hlda}{heteroscedastic \lda{}\xspace}
\newcommand{\Hlda}{Heteroscedastic \lda{}\xspace}
\newcommand{\HLDA}{\textsc{hlda}\xspace}
\hyphenation{hlda}

\newcommand{\mhlda}{multiple \hlda{}\xspace}
\newcommand{\Mhlda}{Multiple \hlda{}\xspace}
\newcommand{\MHLDA}{\textsc{mhlda}\xspace}
\hyphenation{mhlda}

\newcommand{\mlda}{multiple \lda{}\xspace}
\newcommand{\Mlda}{Multiple \lda{}\xspace}
\newcommand{\MLDA}{\textsc{mlda}\xspace}
\hyphenation{mlda}

\newcommand{\VTLN}{\textsc{vtln}\xspace}
\newcommand{\Vtln}{Vocal tract length normalisation\xspace}
\newcommand{\vtln}{vocal tract length normalisation\xspace}

% Noise-robustness techniques and such

\newcommand{\dft}{discrete Fourier transform\xspace}
\newcommand{\Dft}{Discrete Fourier transform\xspace}
\newcommand{\DFT}{\textsc{dft}\xspace}

\newcommand{\dct}{discrete cosine transform\xspace}
\newcommand{\Dct}{Discrete cosine transform\xspace}
\newcommand{\DCT}{\textsc{dct}\xspace}

\newcommand{\mfcc}{Mel-frequency cepstral coefficient\xspace}
\newcommand{\Mfcc}{\mfcc}
\newcommand{\MFCC}{\textsc{mfcc}\xspace}
\newcommand{\mfccs}{{\mfcc}s\xspace}
\newcommand{\Mfccs}{{\Mfcc}s\xspace}
\newcommand{\MFCCs}{{\MFCC}s\xspace}
\hyphenation{mfcc}
\hyphenation{mfccs}

\newcommand{\hmm}{hidden Markov model\xspace}
\newcommand{\Hmm}{Hidden Markov model\xspace}
\newcommand{\HMM}{\textsc{hmm}\xspace}
\newcommand{\hmms}{{\hmm}s\xspace}
\newcommand{\Hmms}{{\Hmm}s\xspace}
\newcommand{\HMMs}{{\HMM}s\xspace}
\hyphenation{hmm}
\hyphenation{hmms}

\newcommand{\gmm}{Gaussian mixture model\xspace}
\newcommand{\Gmm}{\gmm}
\newcommand{\GMM}{\textsc{gmm}\xspace}
\newcommand{\gmms}{{\gmm}s\xspace}
\newcommand{\Gmms}{{\Gmm}s\xspace}
\newcommand{\GMMs}{{\GMM}s\xspace}
\hyphenation{gmm}
\hyphenation{gmms}

\newcommand{\igmm}{infinite \gmm}
\newcommand{\iGMM}{infinite \GMM}
\newcommand{\Igmm}{Infinite \gmm}
\newcommand{\IGMM}{\textsc{igmm}\xspace}
\newcommand{\igmms}{{\igmm}s\xspace}
\newcommand{\iGMMs}{{\iGMM}s\xspace}
\newcommand{\Igmms}{{\Igmm}s\xspace}
\newcommand{\IGMMs}{{\IGMM}s\xspace}
\hyphenation{igmm}
\hyphenation{igmms}

\newcommand{\ihmm}{infinite \hmm}
\newcommand{\iHMM}{infinite \HMM}
\newcommand{\Ihmm}{Infinite \hmm}
\newcommand{\IHMM}{\textsc{ihmm}\xspace}
\newcommand{\ihmms}{{\ihmm}s\xspace}
\newcommand{\iHMMs}{{\iHMM}s\xspace}
\newcommand{\Ihmms}{{\Ihmm}s\xspace}
\newcommand{\IHMMs}{{\IHMM}s\xspace}

\newcommand{\mog}{mixture of Gaussians\xspace}
\newcommand{\Mog}{Mixture of Gaussians\xspace}
\newcommand{\MOG}{\textsc{m}o\textsc{g}\xspace}
\newcommand{\mogs}{mixtures of Gaussians\xspace}
\newcommand{\Mogs}{Mixtures of Gaussians\xspace}
\newcommand{\MOGs}{{\MOG}s\xspace}
\hyphenation{mog}
\hyphenation{mogs}

\newcommand{\fst}{finite-state transducer\xspace}
\newcommand{\Fst}{Finite-state transducer\xspace}
\newcommand{\FST}{\textsc{fst}\xspace}
\newcommand{\fsts}{{\fst}s\xspace}
\newcommand{\Fsts}{{\Fst}s\xspace}
\newcommand{\FSTs}{{\FST}s\xspace}

\newcommand{\fsa}{finite-state automaton\xspace}
\newcommand{\Fsa}{Finite-state automaton\xspace}
\newcommand{\FSA}{\textsc{fsa}\xspace}
\newcommand{\fsas}{finite-state automata\xspace}
\newcommand{\Fsas}{Finite-state automata\xspace}
\newcommand{\FSAs}{{\FSA}s\xspace}

\newcommand{\wfst}{weighted {\fst}\xspace}
\newcommand{\Wfst}{Weighted {\fst}\xspace}
\newcommand{\WFST}{\textsc{wfst}\xspace}
\newcommand{\wfsts}{{\wfst}s\xspace}
\newcommand{\Wfsts}{{\Wfst}s\xspace}
\newcommand{\WFSTs}{{\WFST}s\xspace}

\newcommand{\wfsa}{weighted {\fsa}\xspace}
\newcommand{\Wfsa}{Weighted {\fsa}\xspace}
\newcommand{\WFSA}{\textsc{wfsa}\xspace}
\newcommand{\wfsas}{weighted {\fsas}\xspace}
\newcommand{\Wfsas}{Weighted {\fsas}\xspace}
\newcommand{\WFSAs}{{\WFSA}s\xspace}

\newcommand{\crf}{conditional random field\xspace}
\newcommand{\Crf}{Conditional random field\xspace}
\newcommand{\CRF}{\textsc{crf}\xspace}
\newcommand{\crfs}{conditional random fields\xspace}
\newcommand{\Crfs}{Conditional random fields\xspace}
\newcommand{\CRFs}{\textsc{crf}s\xspace}

\newcommand{\svm}{support vector machine\xspace}
\newcommand{\Svm}{Support vector machine\xspace}
\newcommand{\SVM}{\textsc{svm}\xspace}
\newcommand{\svms}{{\svm}s\xspace}
\newcommand{\Svms}{{\Svm}s\xspace}
\newcommand{\SVMs}{{\SVM}s\xspace}

\newcommand{\ssvm}{structured {\svm}\xspace}
\newcommand{\sSVM}{structured {\SVM}\xspace}
\newcommand{\Ssvm}{Structured {\svm}\xspace}
\newcommand{\SSVM}{\textsc{ssvm}\xspace}
\newcommand{\ssvms}{{\ssvm}s\xspace}
\newcommand{\sSVMs}{{\sSVM}s\xspace}
\newcommand{\Ssvms}{{\Ssvm}s\xspace}
\newcommand{\SSVMs}{{\SSVM}s\xspace}

\newcommand{\spr}{single-pass retraining\xspace}
\newcommand{\Spr}{Single-pass retraining\xspace}
\newcommand{\SPR}{\textsc{spr}\xspace}
\newcommand{\spred}{single-pass retrained\xspace}
\newcommand{\Spred}{Single-pass retrained\xspace}


\newcommand{\mmse}{minimum mean square error\xspace}
\newcommand{\Mmse}{Minimum mean square error\xspace}
\newcommand{\MMSE}{\textsc{mmse}\xspace}
\hyphenation{mmse}

\newcommand{\mbfe}{model-based feature enhancement\xspace}
\newcommand{\Mbfe}{Model-based feature enhancement\xspace}
\newcommand{\MBFE}{\textsc{mbfe}\xspace}

\newcommand{\SPLICE}{\textsc{splice}\xspace}

\newcommand{\vts}{vector Taylor series\xspace}
\newcommand{\Vts}{Vector Taylor series\xspace}
\newcommand{\VTS}{\textsc{vts}\xspace}

\newcommand{\vat}{\VTS adaptive training\xspace}
\newcommand{\Vat}{\vat}
\newcommand{\VAT}{\textsc{vat}\xspace}

\newcommand{\dvat}{discriminative \VTS adaptive training\xspace}
\newcommand{\Dvat}{Discriminative \VTS adaptive training\xspace}
\newcommand{\DVAT}{\textsc{dvat}\xspace}

\newcommand{\cta}{continuous time approximation\xspace}
\newcommand{\Cta}{Continuous time approximation\xspace}
\newcommand{\CTA}{\textsc{cta}\xspace}
\hyphenation{cta}

\newcommand{\jud}{joint uncertainty decoding\xspace}
\newcommand{\Jud}{Joint uncertainty decoding\xspace}
\newcommand{\JUD}{\textsc{jud}\xspace}

\newcommand{\pmc}{parallel model combination\xspace}
\newcommand{\Pmc}{Parallel model combination\xspace}
\newcommand{\PMC}{\textsc{pmc}\xspace}

\newcommand{\dpmc}{data-driven parallel model combination\xspace}
\newcommand{\Dpmc}{Data-driven parallel model combination\xspace}
\newcommand{\DPMC}{\textsc{dpmc}\xspace}
\hyphenation{dpmc}

\newcommand{\idpmc}{iterative data-driven parallel model combination\xspace}
\newcommand{\Idpmc}{Iterative data-driven parallel model combination\xspace}
\newcommand{\IDPMC}{\textsc{idpmc}\xspace}
\hyphenation{idpmc}

\newcommand{\ut}{unscented transformation\xspace}
\newcommand{\Ut}{Unscented transformation\xspace}
\newcommand{\UT}{\textsc{ut}\xspace}

\newcommand{\stcm}{semi-tied covariance matrices\xspace}
\newcommand{\Stcm}{Semi-tied covariance matrices\xspace}
\newcommand{\pstcm}{predictive semi-tied covariance matrices\xspace}
\newcommand{\Pstcm}{Predictive semi-tied covariance matrices\xspace}

\newcommand{\pst}{predictive semi-tied\xspace}
\newcommand{\Pst}{Predictive semi-tied\xspace}
\newcommand{\PST}{\textsc{pst}\xspace}

\newcommand{\pcmllr}{predictive \cmllr}
\newcommand{\Pcmllr}{Predictive \cmllr}
\newcommand{\PCMLLR}{\textsc{pcmllr}\xspace}

\newcommand{\ncmllr}{noisy \cmllr}
\newcommand{\Ncmllr}{Noisy \cmllr}
\newcommand{\NCMLLR}{\textsc{ncmllr}\xspace}
\hyphenation{ncmllr}

\newcommand{\pncmllr}{predictive \ncmllr}
\newcommand{\Pncmllr}{Predictive \ncmllr}
\newcommand{\PNCMLLR}{\textsc{pncmllr}\xspace}
\hyphenation{pncmllr}


% Tools

\newcommand{\wer}{word error rate\xspace}
\newcommand{\Wer}{Word error rate\xspace}
\newcommand{\WER}{\textsc{wer}\xspace}
\newcommand{\wers}{{\wer}s\xspace}
\newcommand{\Wers}{{\Wer}s\xspace}
\newcommand{\WERs}{{\WER}s\xspace}

\newcommand{\ser}{sentence error rate\xspace}
\newcommand{\Ser}{Sentence error rate\xspace}
\newcommand{\SER}{\textsc{ser}\xspace}
\newcommand{\sers}{{\ser}s\xspace}
\newcommand{\Sers}{{\Ser}s\xspace}
\newcommand{\SERs}{{\SER}s\xspace}

\newcommand{\snr}{signal-to-noise ratio\xspace}
\newcommand{\Snr}{Signal-to-noise ratio\xspace}
\newcommand{\SNR}{\textsc{snr}\xspace}
\newcommand{\snrs}{{\snr}s\xspace}
\newcommand{\Snrs}{{\Snr}s\xspace}
\newcommand{\SNRs}{{\SNR}s\xspace}


\newcommand{\htk}{Hidden Markov Model Toolkit\xspace}
\newcommand{\Htk}{Hidden Markov Model Toolkit\xspace}
\newcommand{\HTK}{\textsc{htk}\xspace}

\newcommand{\SCARF}{\textsc{scarf}\xspace}
\newcommand{\ETSI}{\textsc{etsi}\xspace}

% Databases
%\newcommand{\rm}{Resource Management\xspace}
%\newcommand{\Rm}{\rm}
\newcommand{\RM}{\textsc{rm}\xspace}

\newcommand{\AURORA}{\textsc{aurora}\xspace}

\newcommand{\NOISEX}{\textsc{noisex}\xspace}

\newcommand{\TIDIGITS}{\textsc{tidigits}\xspace}

\newcommand{\DARPA}{\textsc{darpa}\xspace}

\newcommand{\NIST}{\textsc{nist}\xspace}

% Projects

\newcommand{\RREAP}{\textsc{r\textsuperscript{2}eap}\xspace}

% Conferences
\newcommand{\IEEE}{\textsc{ieee}\xspace}
\newcommand{\ICASSP}{\textsc{icassp}\xspace}



==> BDL_poster/math_notation.tex <==
\usepackage{keyval}
\usepackage{ifthen}
\usepackage{twoopt}

% Notation

\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\DefinedAs}{\triangleq}
\newcommand{\SetTo}{:=}
\newcommand{\ApproximatedAs}{\simeq}

\newcommand{\ExpectationSymbol}{\mathcal{E}}

% Spaces
\newcommand{\qqquad}{\qquad\qquad}
\newcommand{\qqqquad}{\qqquad\qqquad}

% General notation
\newcommand{\Parentheses}[2][]{\Delimiters[#1]{(}{#2}{)}}
\newcommand{\SquareBrackets}[2][]{\Delimiters[#1]{[}{#2}{]}}
\newcommand{\CurlyBrackets}[2][]{\Delimiters[#1]{\{}{#2}{\}}}
\newcommand{\AngleBrackets}[2][]{\Delimiters[#1]{\langle}{#2}{\rangle}}

\newcommand{\MidBar}[3][]{\Separator[#1]{#2}{|}{#3}}
\newcommand{\MidDoubleBar}[3][]{\Separator[#1]{#2}{\|}{#3}}
\newcommand{\MidBarP}[3][]{\Parentheses[#1]{\MidBar[#1]{#2}{#3}}}

\newcommand{\Given}[3][]{\MidBar[#1]{#2}{#3}}
\newcommand{\GivenP}[3][]{\MidBarP[#1]{#2}{#3}}

\newcommand{\Tuple}[2][]{\Parentheses[#1]{#2}}

% Operations
\newcommand{\Convolution}{*}
\newcommand{\Absolute}[2][]{\Delimiters[#1]{\lvert}{#2}{\rvert}}
\newcommand{\Determinant}[2][]{\Absolute[#1]{#2}}
\newcommand{\Norm}[2][]{\Delimiters[#1]{\|}{#2}{\|}}
\newcommand{\InnerProduct}[2]{\left\langle {#1},{#2} \right\rangle}
\newcommand{\Derivative}[2]{\frac{d #1 }{d #2}}
\newcommand{\DerivativeAt}[4]{\left.\frac{d #1 }{d #2 } #3 \right\rvert_{#4}}
\newcommand{\Partial}[2]{\frac{\partial #1 }{\partial #2}}
\newcommand{\PartialAt}[4]{\left.\frac{\partial #1 }{\partial #2 } #3 \right\rvert_{#4}}
\newcommand{\Integral}[2]{\int{#2} d{#1}}
\newcommand{\IntegralFromTo}[4]{\int_{#2}^{#3} {#4} d{#1}}
\newcommand{\OrderUnder}[2][]{O\Parentheses[#1]{#2}}
\newcommand{\OrderExact}[2][]{\Theta \Parentheses[#1]{#2}}
\newcommand{\OrderOver}[2][]{\Omega\Parentheses[#1]{#2}}

% Functions
\newcommand{\Exp}[1]{e^{#1}}
\newcommand{\ElementLog}{\mbox{\textbf{log}}}
\newcommand{\ElementExp}{\mbox{\textbf{exp}}}

\newcommand{\LogP}[2][]{\log\Parentheses[#1]{#2}}
\newcommand{\ElementLogP}[2][]{\ElementLog\Parentheses[#1]{#2}}

\newcommand{\ExpP}[2][]{\exp\Parentheses[#1]{#2}}
\newcommand{\ElementExpP}[2][]{\ElementExp\Parentheses[#1]{#2}}

\newcommand{\ElementTimes}{\circ}

\newcommand{\DeltaFunction}[3][]{\delta \Parentheses[#1]{ #2 = #3 }}
\newcommand{\KLDivergence}[3][]{\mathcal{KL} \Parentheses[#1]{\MidDoubleBar[#1]{#2}{#3}} }
\newcommand{\Entropy}[2][]{\mathcal{H} \Parentheses[#1]{ #2 } }
\newcommand{\CrossEntropy}[3][]{\mathcal{H} \Parentheses[#1]{\MidDoubleBar[#1]{#2}{#3}} }

\newcommand{\Diagonalise}[2][]{\diag \Parentheses[#1]{#2}}

% Vector or matrix
% The column specification works as follows:
% @{\,}         Left margin: \,
% *{#1}{        #1 times (optional parameter, default=1)
%   c@{\,\,}    Margin between entries: \,\,
% }
% @{\!}         Right margin: \,\,\! which is \,

%\newcommand{\Blocks}[2][1]{\left[ \begin{array}{@{\,}*{#1}{c@{\,\,}}@{\!}} #2 \end{array} \right]}
\newcommandtwoopt{\Blocks}[3][NoSizeOrColumns][NoSize]{%
	\ifthenelse{\equal{#1}{NoSizeOrColumns}}{%
		\def\BlocksDelimiterSize{auto}%
		\def\BlocksColumns{1}%
	}{%
		\ifthenelse{\equal{#2}{NoSize}}{%
			% No size given.
			\def\BlocksDelimiterSize{auto}%
			\def\BlocksColumns{#1}%
		}{%
			\def\BlocksDelimiterSize{#1}%
			\def\BlocksColumns{#2}%
		}%
	}%
	\SquareBrackets[\BlocksDelimiterSize]{
		\begin{array}{@{\,}*{\BlocksColumns}{c@{\,\,}}@{\!}}
			#3
		\end{array}
	}
}

% Probability
\newcommand{\Probability}[2][]{P \Parentheses[#1]{#2}}
\newcommand{\ProbabilityGiven}[3][]{P \Parentheses[#1]{\MidBar[#1]{#2}{#3}}}
\newcommand{\ProbabilityDistribution}[2][p]{#1\Parentheses{#2}}
%\newcommand{\ProbabilityDistributionGiven}[3][p]{#1 \Parentheses{\MidBar{#2}{#3}}}
\newcommand{\Expectation}[2][]{\ExpectationSymbol \CurlyBrackets[#1]{#2}}
\newcommand{\ExpectationUnder}[3][]{\ExpectationSymbol_{#2} \CurlyBrackets[#1]{#3}}
\newcommand{\ExpectationGiven}[3][]{\ExpectationSymbol \CurlyBrackets[#1]{\MidBar[#1]{#2}{#3}}}

\newcommandtwoopt{\ProbabilityDistributionGiven}[4][p][]{#1 \Parentheses[#2]{\MidBar[#2]{#3}{#4}}}

\newcommand{\DiracDelta}[2][]{\delta \Parentheses[#1]{#2}}
\newcommand{\KroneckerDelta}[2]{\delta \Parentheses{#1 - #2}}

%\newcommand{\UniformSymbol}{\mathcal{U}}
%\newcommand{\Uniform}[3][]{\UniformSymbol\Parentheses[#1]{#2, #3}}
\newcommand{\UniformSymbol}{\mathrm{Unif}}
\newcommand{\Uniform}[3][]{\UniformSymbol\SquareBrackets[#1]{#2, #3}}

\newcommand{\NormalSymbol}{\mathcal{N}}
\newcommand{\NormalV}[4][]{\NormalSymbol \Parentheses[#1]{%
    #2 ;\, #3 , \, #4%
}}
% \Normal[size][variable]{mean}{covariance}
% \Normal[variable]{mean}{covariance}
% \Normal{mean}{covariance}
\newcommandtwoopt{\Normal}[4][NoSizeNorVariable][NoSize]{%
	\ifthenelse{\equal{#1}{NoSizeNorVariable}}{%
		\def\NormalDelimiterSize{auto}%
		\def\NormalVariable{}%
	}{%
		\ifthenelse{\equal{#2}{NoSize}}{%
			% No size given.
			\def\NormalDelimiterSize{auto}%
			\def\NormalVariable{#1}%
		}{%
			\def\NormalDelimiterSize{#1}%
			\def\NormalVariable{#2}%
		}%
	}%
	\ifthenelse{\equal{\NormalVariable}{}}{%
	    \NormalSymbol %
	    \Parentheses[\NormalDelimiterSize]{#3, #4}%
    }{%
        \NormalV[\NormalDelimiterSize]{\NormalVariable}{#3}{#4}%
%		\NormalVariable \,;\, #3 \, , \, #4%
	}%
}



% Variable size delimiters

% \Delimiters[Bigg]{(}{text}{)}
\newcommand{\Delimiters}[4][auto]{%
	\ifthenelse{\equal{#1}{normal}}{%
		#2%
		#3%
		#4
	}{%
	\ifthenelse{\equal{#1}{big}}{%
		\big#2%
		#3%
		\big#4%
	}{%
	\ifthenelse{\equal{#1}{Big}}{%
		\Big#2%
		#3%
		\Big#4%
	}{%
	\ifthenelse{\equal{#1}{bigg}}{%
		\bigg#2%
		#3%
		\bigg#4%
	}{%
	\ifthenelse{\equal{#1}{Bigg}}{%
		\Bigg#2%
		#3%
		\Bigg#4%
	}{%
	    % Somehow the automatic setting for delimiter height adds \,
	    % around the delimiters. Undo with \!
		\!\left#2%
		#3%
		% There is sometimes space behind \right#4, but this is usually
		% no a problem, and there is no space when followed by & in an align
		% environment, which is the most common situation.
		% Therefore, the negative space here is commented out:
		\right#4%\!%
	}}}}}%
}

% \Separator[Bigg]{text}{\|}{text}
\newcommand{\Separator}[4][auto]{%
	\ifthenelse{\equal{#1}{normal}}{%
		#2%
		#3%
		#4
	}{%
	\ifthenelse{\equal{#1}{big}}{%
		#2%
		\big#3%
		#4%
	}{%
	\ifthenelse{\equal{#1}{Big}}{%
		#2%
		\Big#3%
		#4%
	}{%
	\ifthenelse{\equal{#1}{bigg}}{%
		#2%
		\bigg#3%
		#4%
	}{%
	\ifthenelse{\equal{#1}{Bigg}}{%
		#2%
		\Bigg#3%
		#4%
	}{%
		\!\left.%
		#2%
		\vphantom{#4}%
		\right#3\!%
		#4%
	}}}}}%
}

% Symbols

\newcommand{\NaturalNumbers}{\mathbb{N}}

\makeatletter

% If #1 is Latin, #2{#1}{<uppercase version of #1>}
% If #1 is Greek, #3{#1}{<uppercase version of #1>}
\newcommand{\ApplyLatinGreek}[3]{%
	\ifthenelse{\equal{#1}{\alpha}}{%
		#3{\alpha}{A}%
	}{%
	\ifthenelse{\equal{#1}{\eta}}{%
		#3{\eta}{H}%
	}{%
	\ifthenelse{\equal{#1}{\theta}}{%
		#3{\theta}{\Theta}%
	}{%
	\ifthenelse{\equal{#1}{\lambda}}{%
		#3{\lambda}{\Lambda}%
	}{%
	\ifthenelse{\equal{#1}{\mu}}{%
		#3{\mu}{\Mu}%
	}{%
	\ifthenelse{\equal{#1}{\sigma}}{%
		#3{\sigma}{\Sigma}%
	}{%
	\ifthenelse{\equal{#1}{\phi}}{%
		#3{\phi}{\Phi}%
	}{%
	\ifthenelse{\equal{#1}{\psi}}{%
		#3{\psi}{\Psi}%
	}{%
	\ifthenelse{\equal{#1}{\omega}}{%
		#3{\omega}{\Omega}%
	}{%
		#2{#1}{\MakeUppercase{#1}}%
	}}}}}}}}}%
}

\newcommand{\mathbfFirst}[2]{\mathbf{#1}}
\newcommand{\bmFirst}[2]{\bm{#1}}
\newcommand{\Second}[2]{#2}
\newcommand{\mathbfSecond}[2]{\mathbf{#2}}
\newcommand{\bmSecond}[2]{\bm{#2}}

% Turn a symbol into an uppercase version even if it's Greek.
\newcommand{\SequenciseSymbol}[1]{%
%    \ApplyLatinGreek{#1}{\Second}{\Second}%
    \ApplyLatinGreek{#1}{\mathbfFirst}{\bmFirst}%
}

% Turn a symbol into an uppercase bold version even if it's Greek.
\newcommand{\MatriciseSymbol}[1]{%
    \ApplyLatinGreek{#1}{\mathbfSecond}{\bmSecond}%
}

% Turn a symbol into an bold version even if it's Greek.
\newcommand{\VectoriseSymbol}[1]{%
    \ApplyLatinGreek{#1}{\mathbfFirst}{\bmFirst}%
}

% Turn a symbol into an uppercase version even if it's Greek.
\newcommand{\CountiseSymbol}[1]{%
    \ApplyLatinGreek{#1}{\Second}{\Second}%
}

% Turn a symbol into a capitalised caligraphic version.
\newcommand{\AggregatiseSymbol}[1]{%
	\mathcal{\MakeUppercase{#1}}%
}

\define@key{symbol}{Matrix}[]{%
	\def\symbol@type{\MatriciseSymbol}%
}
\define@key{symbol}{Sequence}[]{%
	\def\symbol@type{\SequenciseSymbol}%
}
\define@key{symbol}{Vector}[]{%
	\def\symbol@type{\VectoriseSymbol}%
}
\define@key{symbol}{Scalar}[]{%
	\def\symbol@type{}%
}
\define@key{symbol}{Count}[]{%
	\def\symbol@type{\CountiseSymbol}%
}
\define@key{symbol}{Aggregate}[]{%
	\def\symbol@type{\AggregatiseSymbol}%
}
\define@key{symbol}{Space}[]{%
	\def\symbol@type{\AggregatiseSymbol}%
}
\define@key{symbol}{Set}[]{%
	\def\symbol@type{\AggregatiseSymbol}%
}

\newcommand{\FrequentiseSymbol}[1]{%
	\MakeUppercase{#1}%
}

\define@key{symbol}{approximate}[]{%
	\def\symbol@modifier{\widetilde}%
}
\define@key{symbol}{estimate}[]{%
	\def\symbol@modifier{\hat}%
}
\define@key{symbol}{normalised}[]{%
	\def\symbol@modifier{\overline}%
}
\define@key{symbol}{resampled}[]{%
	\def\symbol@modifier{\hat}%
}

\define@key{symbol}{iteration}[\Iteration]{%
	\patchcommand\symbol@superscriptfirst{}{(#1)}%
}
\define@key{symbol}{number}[i]{%
	\patchcommand\symbol@superscriptfirst{}{(#1)}%
}

\define@key{symbol}{inverse}[{-1}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
\define@key{symbol}{square}[{2}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
\define@key{symbol}{cube}[{3}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
\define@key{symbol}{transpose}[\mathsf{T}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
% An inverse and a transpose at once: ^{-T}
\define@key{symbol}{inverseTranspose}[\mathsf{-T}]{%
	\patchcommand\symbol@superscriptsecond{}{#1}%
}
% Hack to keep T's from floating off into space
\define@key{symbol}{innerTranspose}[\mathsf{T}]{%
	\patchcommand\symbol@superscriptsecond{}{\mathllap{#1}}%
}

\define@key{symbol}{index}[\Index]{%
	\patchcommand\symbol@subscriptsecond{}{#1}%
}

\newcommand{\Symbol}[3][]{%
	%%%%% Initialise variables
	\def\symbol@order{}%
	\def\symbol@superscriptfirst{}%
	\def\symbol@superscriptsecond{}%
	\def\symbol@subscriptfirst{}%
	\def\symbol@subscriptfirst@previous{}%
	\def\symbol@subscriptsecond{}%
	\def\symbol@type{}%
	\def\symbol@modifier{}%
	\def\symbol@following{}%
	% Defaults
	\setkeys{symbol}{#1}%
	\setkeys{symbol}{#3}%
	\def\symbol@appearance{\begingroup%
	    \symbol@modifier{\symbol@type{#2}}\endgroup%
	}%
	\patchcommand\symbol@superscriptfirst{\symbol@order}{}%
	%%%%%%% Super- and subscripts
	\ifthenelse{\equal\symbol@superscriptfirst{}}{%
		% No entry for \symbol@superscriptfirst;
		% move \symbol@superscriptsecond to \symbol@superscriptfirst.
		\let\symbol@superscriptsecondcopy\symbol@superscriptsecond%
		\patchcommand\symbol@superscriptfirst{}{\symbol@superscriptsecondcopy}%
		\def\symbol@superscriptsecond{}%
	}{}%
	\ifthenelse{\equal\symbol@subscriptfirst{}}{%
		% No entry for \symbol@subscriptfirst
		% move \symbol@subscriptsecond to \symbol@subscriptfirst.
		\let\symbol@subscriptsecondcopy\symbol@subscriptsecond%
		\patchcommand\symbol@subscriptfirst{}{\symbol@subscriptsecondcopy}%
		\def\symbol@subscriptsecond{}%
	}{}%
	\ifthenelse{\equal{\symbol@superscriptsecond}{}}%
	{%
		% If \symbol@superscriptsecond is empty
		\ifthenelse{\not{\equal{\symbol@subscriptsecond}{}}}%
		{%
			% use a comma
			\let\symbol@subscriptsecondcopy\symbol@subscriptsecond%
			\patchcommand\symbol@subscriptfirst{}{,\symbol@subscriptsecondcopy}%
			\def\symbol@subscriptsecond{}%
		}{}%
	}{%
		% If \symbol@superscriptsecond is non-empty
		\ifthenelse{\not{\equal{\symbol@subscriptsecond}{}}}%
		{%
			% use a comma
			\patchcommand\symbol@subscriptfirst{}{,}%
		}{}%
	}%
	%%%%%%% Output
	\def\symbol@first{%
		{\symbol@appearance}%
    	{\symbol@following}%
			\ifthenelse{\equal{\symbol@subscriptfirst}{}}{}%
				{_{\symbol@subscriptfirst}}%
			\ifthenelse{\equal{\symbol@superscriptfirst}{}}{}%
				{^{\symbol@superscriptfirst}}%
		}%
	\ifthenelse{\equal{\symbol@subscriptsecond\symbol@superscriptsecond}{}}%
		% No second-level entries
%		{\mbox{$\symbol@first$}}%
		{\symbol@first}%
		{%
			{\mbox{$\symbol@first$}}%
			\ifthenelse{\equal{\symbol@subscriptsecond}{}}{}%
				{_{\symbol@subscriptsecond}}%
			\ifthenelse{\equal{\symbol@superscriptsecond}{}}{}%
				{^{\symbol@superscriptsecond}}%
		}%
}

\makeatother

\newcommand{\Nothing}[1][]{%
	\Symbol[Matrix]{}{#1}%
}

\newcommand{\TransposeOf}[1]{%
	\Symbol{{#1}}{transpose}%
}
\newcommand{\InverseOf}[1]{%
	\Symbol{{#1}}{inverse}%
}
\newcommand{\SquareOf}[1]{%
	\Symbol{#1}{square}%
}
\newcommand{\IndexOf}[3][]{%
	\Symbol{#2}{index=#3, #1}%
}

\newcommand{\Zeros}[1][]{%
	\Symbol[Vector]{0}{#1}%
}
\newcommand{\Ones}[1][]{%
	\Symbol[Vector]{1}{#1}%
}

\newcommand{\DistributionSymbol}{p}
\newcommand{\Distribution}[1][]{%
	\Symbol{\DistributionSymbol}{#1}%
}



==> BDL_poster/symbols.tex <==
\usepackage{keyval}
\usepackage{patchcmd}
\usepackage{ifthen}
\usepackage{bm}

\input{math_notation}

%%%%%%%%%%%%
% Non-general things

%\usepackage{tipa}
%\newcommand{\PhoneExample}{\textipa{\ae}}
%% For retaining \! in math mode:
%\tipasafemode
\newcommand{\PhoneExampleOne}{ei}%\textsc{i}}
\newcommand{\PhoneExampleTwo}{t}

\newcommand{\WordIndexSymbol}{i}
\newcommand{\WordIndex}[1][]{%
	\Symbol[Scalar]{\WordIndexSymbol}{#1}%
}
\newcommand{\VocabularyWordSymbol}{v}
\newcommand{\VocabularyWord}[1][]{%
	\Symbol[Scalar]{\VocabularyWordSymbol}{#1}%
}
\newcommand{\VocabularyIndexSymbol}{j}
\newcommand{\VocabularyIndex}[1][]{%
	\Symbol[Scalar]{\VocabularyIndexSymbol}{#1}%
}

\newcommand{\SegmentSymbol}{s}
\newcommand{\Segment}[1][]{%
	\Symbol[Scalar]{\SegmentSymbol}{#1}%
}

\newcommand{\StartNodeName}{\text{start}}
\newcommand{\EndNodeName}{\text{end}}
\DeclareMathOperator*{\Forward}{forwd}
\DeclareMathOperator*{\Backward}{backwd}

\newcommand{\SemiringPlus}{\oplus}
\newcommand{\SemiringTimes}{\otimes}

\newcommand{\LanguageModelSize}{L}


\makeatletter

\define@key{symbol}{Automaton}[]{%
	\def\symbol@type{\AggregatiseSymbol}%
}

\makeatother

\newcommand{\GradientSymbol}{\nabla}
\newcommand{\Gradient}[1][]{%
	\Symbol[Scalar]{\GradientSymbol}{#1}%
}

\newcommand{\TransducerComposition}{\circ}

\newcommand{\SubPhoneAutomatonSymbol}{s}
\newcommand{\SubPhoneAutomaton}[1][]{%
	\Symbol[Automaton]{\SubPhoneAutomatonSymbol}{#1}%
}

\newcommand{\ObservationTransducerSymbol}{o}
\newcommand{\ObservationTransducer}[1][]{%
	\Symbol[Automaton]{\ObservationTransducerSymbol}{#1}%
}

\newcommand{\TrellisTransducerSymbol}{t}
\newcommand{\TrellisTransducer}[1][]{%
	\Symbol[Automaton]{\TrellisTransducerSymbol}{#1}%
}

\newcommand{\ArcSymbol}{e}
\newcommand{\Arc}[1][]{%
	\Symbol[Scalar]{\ArcSymbol}{#1}%
}

\newcommand{\PathSymbol}{\pi}
%\newcommand{\Path}{\Arc[Sequence]}
\newcommand{\Path}[1][]{%
	\Symbol[Scalar]{\PathSymbol}{#1}%
}

\newcommand{\WeightSymbol}{\sigma}
\newcommand{\Weight}[1][]{%
	\Symbol[Scalar]{\WeightSymbol}{#1}%
}
\newcommand{\WeightOf}[3][]{\Weight \SquareBrackets[#1]{ #2 ; #3}}

\newcommand{\PosteriorSymbol}{\gamma}
\newcommand{\Posterior}[1][]{%
	\Symbol[Scalar]{\PosteriorSymbol}{#1}%
}

\newcommand{\StartNodeSymbol}{p}
\newcommand{\StartNode}[1][]{%
	\Symbol[Scalar]{\StartNodeSymbol}{#1}%
}
\newcommand{\StartNodeOf}[2][]{\StartNode \SquareBrackets[#1]{ #2 }}

\newcommand{\EndNodeSymbol}{n}
\newcommand{\EndNode}[1][]{%
	\Symbol[Scalar]{\EndNodeSymbol}{#1}%
}
\newcommand{\EndNodeOf}[2][]{\EndNode \SquareBrackets[#1]{ #2 }}

\newcommand{\SemiringZero}{\overline 0}
\newcommand{\SemiringOne}{\overline 1}

\newcommand{\InputSymbolSymbol}{e}
\newcommand{\InputSymbol}[1][]{%
	\Symbol[Scalar]{\InputSymbolSymbol}{#1}%
}

\newcommand{\OutputSymbolSymbol}{o}
\newcommand{\OutputSymbol}[1][]{%
	\Symbol[Scalar]{\OutputSymbolSymbol}{#1}%
}

\newcommand{\LikelihoodSymbol}{\ell}
\newcommand{\Likelihood}[1][]{%
	\Symbol[Scalar]{\LikelihoodSymbol}{#1}%
}

\newcommand{\LikelihoodOf}[3][]{\Likelihood \SquareBrackets[#1]{ #2 ; #3}}
\newcommand{\LikelihoodOfAll}[2][]{\Likelihood \Parentheses[#1]{#2}}
\newcommand{\LikelihoodGiven}[3][]{\Likelihood \Parentheses[#1]{ #2 ; #3}}


%%%%%%%%%%%%%%

\newcommand{\TimeSymbol}{t}
\newcommand{\OtherTimeSymbol}{\tau}
\newcommand{\IndexSymbol}{i}
\newcommand{\WordSymbol}{w}

\newcommand{\VariableSymbol}{v}
\newcommand{\FactorSymbol}{f}
\newcommand{\FeatureSymbol}{\phi}
\newcommand{\NormalisationSymbol}{Z}

\newcommand{\ParameterSymbol}{\alpha}
\newcommand{\GenerativeParameterSymbol}{\lambda}

\newcommand{\StateSymbol}{s}
\newcommand{\ObservationSymbol}{o}

\newcommand{\EmptySymbol}{\epsilon}

\DeclareMathOperator*{\ParentsSymbol}{pa}

%%%%%% Implementations

\newcommand{\Parents}[1]{\ParentsSymbol \Parentheses{#1}}

\newcommand{\Time}[1][]{%
	\Symbol[Scalar]{\TimeSymbol}{#1}%
}
\newcommand{\TotalTime}[1][]{%
	\Symbol[Count]{\TimeSymbol}{#1}%
}
\newcommand{\TimeNum}[1][]{%
	\Symbol[Count]{\TimeSymbol}{#1}%
}
\newcommand{\OtherTime}[1][]{%
	\Symbol[Scalar]{\OtherTimeSymbol}{#1}%
}
\newcommand{\Index}[1][]{%
	\Symbol[Scalar]{\IndexSymbol}{#1}%
}

\newcommand{\Word}[1][]{%
	\Symbol[Scalar]{\WordSymbol}{#1}%
}

\newcommand{\State}[1][]{%
	\Symbol[Scalar]{\StateSymbol}{#1}%
}
\newcommand{\Observation}[1][]{%
	\Symbol[Scalar]{\ObservationSymbol}{#1}%
}

\newcommand{\Variable}[1][]{%
	\Symbol[Scalar]{\VariableSymbol}{#1}%
}
\newcommand{\Factor}[1][]{%
	\Symbol[Scalar]{\FactorSymbol}{#1}%
}
\newcommand{\Feature}[1][]{%
	\Symbol[Scalar]{\FeatureSymbol}{#1}%
}

\newcommand{\Normalisation}[1][]{%
	\Symbol[Scalar]{\NormalisationSymbol}{#1}%
}

\newcommand{\Parameter}[1][]{%
	\Symbol[Scalar]{\ParameterSymbol}{#1}%
}
\newcommand{\GenerativeParameter}[1][]{%
	\Symbol[Scalar]{\GenerativeParameterSymbol}{#1}%
}

\makeatletter

%\define@key{symbol}{velocity}[\mathsf{\Delta}]{%
\define@key{symbol}{velocity}[\Delta]{%
	\def\symbol@order{#1}%
}
\define@key{symbol}{acceleration}[\Delta^2]{%
	\def\symbol@order{#1}%
}

\define@key{symbol}{time}[\TimeSymbol]{%
	\ifthenelse{\equal{\symbol@subscriptfirst@previous}{symbol}}{%
		\patchcommand\symbol@subscriptfirst{}{_{#1}}%
	}{%
		\patchcommand\symbol@subscriptfirst{}{#1}%
	}%
}

\define@key{symbol}{best}[*]{%
	\patchcommand\symbol@superscriptfirst{}{#1}%
}

\define@key{symbol}{state}[\mathsf{\StateSymbol}]{%
	\patchcommand\symbol@subscriptfirst{}{#1}%
%	\def\symbol@subscriptfirst@previous{symbol}%
}
\define@key{symbol}{observation}[\mathsf{\ObservationSymbol}]{%
	\patchcommand\symbol@subscriptfirst{}{#1}%
	\def\symbol@subscriptfirst@previous{symbol}%
}

\define@key{symbol}{sequential}[\text{\textsf{seq}}]{%
	\patchcommand\symbol@superscriptfirst{}{#1}%
}
\define@key{symbol}{observational}[\text{\textsf{obs}}]{%
	\patchcommand\symbol@superscriptfirst{}{#1}%
}

\makeatother



==> BDL_poster/ucamcolor.tex <==
%--------------------------------------------------------
% Set up the Cambridge University Colours for use with
% xcolor
%--------------------------------------------------------

% Blue palette
% Pantone 284 C
\definecolor{lightBlue}{rgb}{0.4157 0.6784 0.8941}
% Pantone 285 C
\definecolor{coreBlue}{rgb}{0 0.4510 0.8118}
% Pantone 541 C
\definecolor{darkBlue}{rgb}{0 0.2341 0.4471}

% Orange palette
% Pantone 142 C
\definecolor{lightOrange}{rgb}{0.9373 0.7412 0.2784}
% Pantone 158 C
\definecolor{coreOrange}{rgb}{0.8902 0.4471 0.1333}
% Pantone 718 C
\definecolor{darkOrange}{rgb}{0.7843 0.3059 0}

% Green palette
% Pantone 583 C
\definecolor{lightGreen}{rgb}{0.6588 0.7059 0}
% Pantone 369 C
\definecolor{coreGreen}{rgb}{0.3451 0.6510 0.0941}
% Pantone 574 C
\definecolor{darkGreen}{rgb}{0.2627 0.3176 0.1451}

% Purple palette
% Pantone 5215 C
\definecolor{lightPurple}{rgb}{0.7098 0.5765 0.6078}
% Pantone 513 C
\definecolor{corePurple}{rgb}{0.5569 0.1451 0.5529}
% Pantone 669 C
\definecolor{darkPurple}{rgb}{0.2549 0.1765 0.3647}

% Teal palette
% Pantone 557 C
\definecolor{lightTeal}{rgb}{0.6392 0.7569 0.6784}
% Pantone 7466 C
\definecolor{coreTeal}{rgb}{0 0.7020 0.7451}
% Pantone 5473 C
\definecolor{darkTeal}{rgb}{0.0824 0.3961 0.4392}



==> distillation_structured_uncertainty.tex <==
\section{Distillation for Structured Prediction}

The key expression associated with distillation approaches is to train a model with parameters ${\hat{\bm \theta}}$ to emulate the performance of a pretrained model with parameters ${\overline{\bm\theta}}$. This can be viewed as training an initial parameters to model the posterior distribution from  true data distribution ${\tt p}){\tt tr}({\bm x},y)$ where ${\bm x}$ is the observation and $y$ is the class label. In practice there are only samples from this true distribution to train on
\begin{eqnarray*}
{\cal D}
%% =\left\{\{{\bm x}^{(1)},y^{(1)}\},\ldots,{\bm x}^{(N)},y^{(N)}\}\right\}
=
\left\{\{{\bm x}^{(i)},y^{(i)}\}\right\}_{i=1}^N
; \:\:\:\:
y^{(i)}\in\{\omega_1,\ldots,\omega_K\}
\end{eqnarray*}
In terms of standard notation given the training data ${\cal D}$ training can be expressed as
\begin{eqnarray}
{\overline{\bm\theta}} = 
= 
\argmax_{\bm\theta}\left\{
\sum_{i=1}^N
\log\left({\tt P}(y^{(i)}|\bm{x}^{(i)}; {{\bm{\theta}}})\right)
\right\}
\end{eqnarray}
The labels, $y$ from the joint distribution are now discarded, and the posteriors frome the trained model are used to estimate the distilled model parameters ${\hat{\bm\theta}}$
\begin{eqnarray}
{\hat{\bm\theta}} = \argmin_{\bm\theta}\left\{
\sum_{i=1}^N{\tt KL}\big[
{\tt P}(y|\bm{x}^{(i)}; {\overline{\bm{\theta}}})
\big|\big|
{{\tt P}(y|\bm{x}^{(i)}; {{\bm{\theta}}})}
\big]
\right\}
\end{eqnarray}
where
\begin{eqnarray}
{\tt KL}\big[
{\tt P}(y|\bm{x}^{(i)}; {\overline{\bm{\theta}}})
\big|\big|
{{\tt P}(y|\bm{x}^{(i)}; {{\bm{\theta}}})}
\big] = 
\sum_{k=1}^K{\tt P}(y=\omega_k|{\bm x}^{(i)}; {\overline{\bm{\theta}}})\log
\left(
\frac{{\tt P}(y=\omega_k|{\bm x}^{(i)}; {\overline{\bm{\theta}}})}
{{\tt P}(y=\omega_k|{\bm x}^{(i)};{\bm\theta})}
\right)
\end{eqnarray}
When the data is now structured, for example tasks such as speech recognition, speech synthesis and machine translation the joint distribution of the data is more complicated as there are now observations sequences and label sequences. The data distribution can be expressed as~\footnote{Of course $T$ and $L$ vary, but for simplicity this is ignored for notational simplicity.} ${\tt p}_{\tt tr}({\bm x}_{1:T},y_{1:L})$. Again only samples from the true distribution 
\begin{eqnarray*}
{\cal D}
%% =\left\{\{{\bm x}^{(1)},y^{(1)}\},\ldots,{\bm x}^{(N)},y^{(N)}\}\right\}
=
\left\{\{{\bm x}^{(i)}_{1:T},y^{(i)}_{1:L}\}\right\}_{i=1}^N
; \:\:\:\:
y^{(i)}\in\{\omega_1,\ldots,\omega_K\}
\end{eqnarray*}
Again this data can be used to train a standard sequence model with parameters ${\overline{\bm\theta}}$. One optimal difference is that the simple (conditional) maximum likelihood training for unstructured data can use minimum Bayes risk training with an appropriate sequence loss function.  The original implementation of knowledge distillation, or teacher-student training, for this form of model used a simple per sample approximation
\begin{eqnarray}
{\hat{\bm\theta}} = \argmin_{\bm\theta}\left\{
\sum_{i=1}^N\sum_{j=1}^T{\tt KL}\big[
{\tt P}(y|\bm{x}^{(i)}_j; {\overline{\bm{\theta}}})
\big|\big|
{{\tt P}(y|\bm{x}^{(i)}_j; {{\bm{\theta}}})}
\big]
\right\}
\end{eqnarray}
Effectively this has ignored the problem as a sequence problem. Sequence teacher-student training, sequence distillation, aims to address this problem by considering posterior distributions of complete sequences, compressed into a lattice ${\cal L}$ generated from model ${\overline{\bm\theta}}$ for the $i-th$ sample, ${\cal L}|\bm{x}^{(i)}_{1:T}; {\overline{\bm{\theta}}}$. The expression then becomes
\begin{eqnarray}
{\hat{\bm\theta}} = \argmin_{\bm\theta}\left\{
\sum_{i=1}^N{\tt KL}\big[
{\cal L}|\bm{x}^{(i)}_{1:T}; {\overline{\bm{\theta}}}
\big|\big|
{\cal L}|\bm{x}^{(i)}_{1:T}; {\bm{\theta}}
\big]
\right\}
\end{eqnarray}

For these approaches there is no assumption that the complexity of the models is consistent between ${\overline{\bm\theta}}$ and ${\hat{\bm\theta}}$. This distillation can be used to simplify the complexity of the model, yielding speed and memory advantages.

The second application of distillation is to distill an ensemble of models into a single model. Applying standard ensemble distillation
\begin{eqnarray}
{\hat{\bm\theta}} = \argmin_{\bm\theta}\left\{
\sum_{i=1}^N\sum_{m=1}^M{\tt KL}\big[
{\tt p}(y|\bm{x}^{(i)}; {\overline{\bm{\theta}}}^{(m)})
\big|\big|
{\tt p}(y|\bm{x}^{(i)}; {\bm{\theta}})
\big]
\right\}
\end{eqnarray}
where the ensemble of models comprises parameters, $\left\{{\overline{\bm\theta}}^{(m)}\right\}_{m=1}^M$.  As previously mentioned this has ignored the diversity associated with the model. To address this problem ensemble distribution distillation can be used. Here the distribution of the predictions in the ensemble is modelled. Denote the prediction of sample ${\bm x}^{(i)}$ using model ${\overline{\bm\theta}}^{(m)}$ as
\begin{eqnarray}
{\bm\pi}^{(mi)} = \left[
\begin{array}{c}
{\tt P}(y=\omega_1|{\bm x}^{(i)};{\overline{\bm\theta}}^{(m)}) \\
\vdots\\
{\tt P}(y=\omega_K|{\bm x}^{(i)};{\overline{\bm\theta}}^{(m)}) 
\end{array}
\right]; 
\:\:\:\:
{\bm\pi}^{(mi)} \sim {\tt p}_{\pi}({\bm x}^{(i)})
\end{eqnarray}
To model the ensemble distribution these samples can then be used for training the model
\begin{eqnarray}
{\hat{\bm\theta}} = 
\argmin_{\bm\theta}\left\{
\sum_{i=1}^N
{\tt KL}\big[
{\tt p}_{\pi}(\bm{x}^{(i)})
\big|\big|
{\tt p}_{\pi}(\bm{x}^{(i)}; {\bm{\theta}})
\big]
\right\}
\approx
\argmax_{\bm\theta}\left\{
\sum_{i=1}^N
\sum_{m=1}^M
\log\left(
{\tt p}_{\pi}({\bm\pi}^{(mi)} | \bm{x}^{(i)}; {\bm{\theta}})
\right)
\right\}
\end{eqnarray}
This form of model, associated with distributions over distributions, is a prior network. This has the same form as density networks, networks that predict the parameters of parametric distributions, but the form here is a distribution over distributions. Thus
\begin{eqnarray*}
{\tt p}_{\pi}({\bm\pi}^{(mi)} | \bm{x}^{(i)}; {\bm{\theta}})
= {\tt Dir}({\bm\pi}^{(mi)}; {\cal F}_\alpha(\bm{x}^{(i)}; {\bm{\theta}}))
\end{eqnarray*}
where ${\cal F}_\alpha(\bm{x}^{(i)}; {\bm{\theta}})$ yields the appropriate Dirichlet distribution parameters.

Extending this form of distribution to handle structured data is non-trivial. It is possible to extend the notation above to handle lattices
\begin{eqnarray}
{\cal L}^{(mi)} = 
{\cal L}|{\bm x}^{(i)};{\overline{\bm\theta}}^{(m)};
\:\:\:\:
{\cal L}^{(mi)} \sim {\tt p}_{\cal L}({\bm x}^{(i)})
\end{eqnarray}
The challenge is to decide on the appropriate parametric form for ${\tt p}_{\cal L}({\bm x}^{(i)};{\bm\theta})$.

\section{Sequence Distribution Distillation}
The simplest approach to a distribution over the lattice~\footnote{The initial form considered here is a prefix-tree not a lattice.} is to make an additional conditional independence assumption: the distribution over the predicted word distributions is only dependent on the history of words to that point. Thus consider adding a new arc ${\cal A}$ to the lattice having taken word sequence $w_{1:\tau-1}=w_1,\ldots,w_{\tau-1}$ where $w_\tau\in\{\omega_k\}_{k=1}^K$. Initially just consider the scenario where only the word-id information is  considered (so duration and score are not considered). The task is to get the distribution over the predictions for word $w_\tau$. Consider
\begin{eqnarray*}
{\tt p}_{\pi}({{\bm\pi}}_{\tau}|w_{1:\tau-1};{\bm\theta})
\end{eqnarray*}
where
\begin{eqnarray}
{\bm\pi}_{\tau} = \left[
\begin{array}{c}
{\tt P}(y=\omega_1|w_{1:\tau-1}) \\
\vdots\\
{\tt P}(y=\omega_K|w_{1:\tau-1}) 
\end{array}
\right]
\end{eqnarray}

Consider the following form
\begin{eqnarray}
{\tt p}_{\pi}({{\bm\pi}}_{\tau}|w_{1:\tau-1};{\bm\theta})
\approx
{\tt p}_{\pi}({{\bm\pi}}_{\tau}|w_{\tau-1},{\bm\alpha}_{\tau-1};{\bm\theta})
= {\tt Dir}({{\bm\pi}}_{\tau};{\cal F}_\alpha(w_{\tau-1},{\bm\alpha}_{\tau-1};{\bm\theta})
= {\tt Dir}({{\bm\pi}}_{\tau};{\bm\alpha}_{\tau})
\end{eqnarray}
This effectively replaces the standard PMF prediction from an RNN-LM, with a Dirichlet distribution prediction. Following this logic through
\begin{eqnarray}
{\cal F}_\alpha(w_{\tau},{\bm\alpha}_{\tau};{\bm\theta}) \approx
{\cal F}_\alpha(w_{\tau},{\bm h}_{\tau};{\bm\theta}); \:\:\:\:
{\bm h}_{\tau} = {\cal F}_{\tt h}(w_{\tau-1},{\bm h}_{\tau-1};{\bm\theta})
\end{eqnarray}
This form of model can be trained in the same fashion as standard LMs, but now using the distributions that result from an ensemble if language models. Let 
\begin{eqnarray}
{\bm\pi}^{(m)}_{\tau} = \left[
\begin{array}{c}
{\tt P}(y=\omega_1|w_{1:\tau-1};{\bm\theta}^{(m)}) \\
\vdots\\
{\tt P}(y=\omega_K|w_{1:\tau-1};{\bm\theta}^{(m)}) 
\end{array}
\right]
\end{eqnarray}
The optimisation criterion then becomes
\begin{eqnarray}
{\hat{\bm\theta}} = \argmax_{{\bm\theta}}\left\{
\sum_{\tau=1}^L\sum_{m=1}^M\log\left(
{\tt p}_{\pi}({\bm\pi}^{(m)}_{\tau}|w_{1:\tau-1};{\bm\theta})
\right)
\right\}
\end{eqnarray}



==> ensemble_uncertainty.tex <==
\section{Uncertainty Estimation via Ensembles}\label{sec:ensembles}
%%%%FLOW!!!!!!%%%%

In this work we take a Bayesian viewpoint on ensembles, as it yields an elegant probabilistic framework within which interpretable uncertainty estimates can be obtained. The core of the Bayesian approach is to treat the model parameters $\bm{\theta}$ as random variables and place a prior  ${\tt p}(\bm{\theta})$ over them to compute a posterior ${\tt p}(\bm{\theta}|\mathcal{D})$ via Bayes' rule.
% \begin{empheq}{align}
% \begin{split}
%   {\tt p}(\bm{\theta}|\mathcal{D}) &= \frac{{\tt p}(\mathcal{D}|\bm{\theta}){\tt p}(\bm{\theta})}{{\tt p}(\mathcal{D})}
% \end{split}
% \label{eqn:bayesposterior}
% \end{empheq}
However, exact Bayesian inference is intractable for neural networks. It is therefore necessary to consider an explicit or implicit approximation ${\tt q}(\bm{\theta})$ to the true posterior ${\tt p}(\bm{\theta}|\mathcal{D})$ to generate an ensemble of models. A number of different approaches to generating an ensemble of models have been developed, such as Monte-Carlo Dropout~\cite{Gal2016Dropout} and DeepEnsembles~\cite{deepensemble2017}. A full overview is available in~\cite{ashukha2020pitfalls, trust-uncertainty}. 

Consider an ensemble of models $\{{\tt P}(y | \bm{x}; \bm{\theta}^{(m)})\}_{m=1}^M$ sampled from an approximate posterior ${\tt q}(\bm{\theta})$, where each model captures an \emph{unstructured} mapping $\bm{x} \rightarrow y$, where $\bm{x} \in \mathcal{R}^D$ and $y \in \{\omega_1,\cdots,\omega_K\}$. Each of the models ${\tt P}(y|\bm{x}, \bm{\theta}^{(m)})$ yields a \emph{different} estimate of \emph{data uncertainty}. Uncertainty in predictions due to \emph{knowledge uncertainty} is expressed as the level of spread, or `disagreement', of models in the ensemble~\cite{malinin-thesis}. The \emph{predictive posterior} of the ensemble is obtained by taking the expectation with respect to the models in the ensemble:
\begin{empheq}{align}
\begin{split}
{\tt P}(y | \bm{x}, \mathcal{D}) =&\  \mathbb{E}_{{\tt p}(\bm{\theta}|\mathcal{D})}\big[{\tt P}(y | \bm{x} ; \bm{\theta}) \big]
\approx\ \frac{1}{M}\sum_{m=1}^M {\tt P}(y | \bm{x}; \bm{\theta}^{(m)}),\ \bm{\theta}^{(m)} \sim {\tt q}(\bm{\theta})
\end{split}
\end{empheq}
% The entropy of the predictive posterior will be an estimate of \emph{total uncertainty} in predictions:
% \begin{empheq}{align}
% \mathcal{H}\big[{\tt P}(y |  \bm{x}, \mathcal{D})\big] =&\  \mathbb{E}_{{\tt P}(y |  \bm{x},  \mathcal{D})}\big[ -\ln {\tt P}(y | \bm{x},  \mathcal{D}) \big] 
% \end{empheq}
% \emph{Total uncertainty} in the prediction is due to both \emph{data uncertainty} and \emph{knowledge uncertainty}. However, for tasks such as misclassification detection considering the log-likelihood score (SCR) assigned by the predictive posterior to a particular class $\hat \omega$ can yield superior performance as it is more sensitive to the prediction made~\cite{malinin-thesis}:
% \begin{empheq}{align}
% \begin{split}
% \text{SCR} =&\ \ln{\tt P}(y = \hat \omega| \bm{x}, \mathcal{D})
% \end{split}
% \end{empheq}
In certain situations, such as active learning~\cite{batchbald} and out-of-distribution detection, it is desirable to evaluate uncertainty in predictions due to \emph{knowledge uncertainty}. The sources of uncertainty can be decomposed by considering the \emph{mutual information} between $\bm{\theta}$ and the prediction $y$~\cite{mutual-information}:
\begin{empheq}{align}
\begin{split}
\underbrace{\mathcal{I}\big[y, \bm{\theta} | \bm{x}, \mathcal{D}\big]}_{\text{Knowledge Uncertainty}} =&\ \underbrace{\mathcal{H}\big[{\tt P}(y |  \bm{x}, \mathcal{D})\big]}_{\text{Total Uncertainty}} -   \underbrace{\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(y | \bm{x}; \bm{\theta})]\big]}_{\text{Expected Data Uncertainty}}
\end{split}\label{eqn:mi}
\end{empheq}
This is expressed as the difference between the entropy of the predictive posterior and the expected entropy of each model in the ensemble. The former is a measure of \emph{total uncertainty}, while the later is a measure of \emph{expected data uncertainty}. Their difference will be measure of spread of the ensemble and an estimate of \emph{knowledge uncertainty}. It is also possible to consider the \emph{expected pairwise KL-divergence} (EPKL) between models in an ensemble as an alternative measure of diversity:
\begin{empheq}{align}
\begin{split}
\mathcal{K}[y, \bm{\theta}| \bm{x}, \mathcal{D}] =&\ \mathbb{E}_{{\tt q}(\bm{\theta}){\tt q}(\bm{\tilde \theta})}\big[{\tt KL}[{\tt P}(y|\bm{x},\bm{\theta})||{\tt P}(y|\bm{x},\bm{\tilde \theta}) ]\big] \\
=&  \underbrace{-\mathbb{E}_{{\tt P}(y|\bm{x}, \mathcal{D})}\big[\mathbb{E}_{{\tt q}(\bm{\tilde \theta})}[\ln{\tt P}(y|\bm{x}, \bm{\tilde \theta})]\big]}_{\text{Total Uncertainty}} -   \underbrace{\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(y | \bm{x}; \bm{\theta})]\big]}_{\text{Expected Data Uncertainty}}
\end{split}
\label{eqn:epklbayes}
\end{empheq}
where ${\tt q}(\bm{\theta})={\tt q}(\bm{\tilde \theta})$. This measure is an upper bound on the mutual information and also allows \emph{total uncertainty} to be decomposed into \emph{knowledge uncertainty} and \emph{data uncertainty}~\cite{malinin-thesis}. Notably, ~\ref{eqn:mi} and~\ref{eqn:epklbayes} only differ in their estimates of \emph{total uncertainty} differ. 
% We can also examine measures which only consider the probability of the predicted class $ \hat \omega$. Firstly, we can examine the log-likelihood of the predicted token under the predictive posterior:
% \begin{empheq}{align}
% \begin{split}
% \text{SCR} =&\ -\ln{\tt P}(y_l = \hat \omega_l | \bm{y}_{<l}, \bm{X}, \mathcal{D}),\quad \text{eSCR} =\ -\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\ln{\tt P}(y_l = \hat \omega_l | \bm{y}_{<l}, \bm{X}, \bm{\theta})\big]
% \end{split}\label{eqn:token-posterior-score}
% \end{empheq}
% This is a measure of \emph{total uncertainty}. Alternatively, we can consider the expected log-probability assigned by each model in the ensemble.
% This will be a measure of \emph{data uncertainty}. Finally, we can consider the the  mean negative \emph{Point-wise Mutual Information}~\cite{murphy} between the model $\bm{\theta}^{(m)}$ and the prediction $\bm{y}_l$ across all models:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{M} =&\ - \mathbb{E}_{{\tt q}(\bm{\theta})}\underbrace{\Big[\ln\frac{{\tt P}(y = \hat \omega |  \bm{x}, \bm{\theta})}{{\tt P}(y = \hat \omega | \bm{x}, \mathcal{D})}\Big]}_{\text{Pointwise Mutual Information}}
% =\ \text{eSCR} - \text{SCR} \geq 0
% \end{split}\label{eqn:token-npmi}
% \end{empheq}
% This difference will be a measure of ensemble diversity, and therefore \emph{knowledge uncertainty}.






% First, let's consider the entropy of as single model in the ensemble at an input $\bm{x}$:
% \begin{empheq}{align}
% \begin{split}
%  \mathcal{H}\big[{\tt P}(y | \bm{x}; \bm{\theta})\big]
% =&\ \mathbb{E}_{{\tt P}(y |  \bm{x}; \bm{\theta})}\big[ -\ln {\tt P}(y | \bm{x}; \bm{\theta}) \big] 
% \end{split}
% \end{empheq}
% This will be an estimate of \emph{data uncertainty}, or uncertainty due to the natural complexity of the data~\cite{malinin-thesis}.

==> leftovers.tex <==
% \subsection{Sequence-level Uncertainty Estimates}

% % \begin{empheq}{align}
% % \begin{split}
% % \mathcal{H}[{\tt P}(\bm{y} | \bm{x}, \bm{\theta})] =&\ \mathbb{E}_{{\tt P}(\bm{y} | \bm{x}, \bm{\theta})}\big[\ln {\tt P}(\bm{y} | \bm{x}, \bm{\theta})\big]
% % \end{split}
% % \end{empheq}

% As discussed in section~\ref{sec:struct-uncertainty}, one can obtain measures of \emph{total}, \emph{data} and \emph{knowledge uncertainty} at the \emph{sequence level} by considering the mutual information between the sequence $\bm{y}$ and the parameters $\bm{\theta}$:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{I}\big[\bm{y}, \bm{\theta} |  \bm{x}, \mathcal{D}\big]  =&\ \mathbb{E}_{{\tt q}(\bm{\theta})} \big[{\tt KL}[{\tt P}(\bm{y}|\bm{x}, \bm{\theta})\|{\tt P}(\bm{y} | \bm{x}, \mathcal{D})]\big] \\
% =&\  \mathbb{E}_{{\tt q}(\bm{\theta})} \Big[\mathbb{E}_{{\tt P}(\bm{y}|\bm{x}, \bm{\theta})}\Big[\ln\frac{{\tt P}(\bm{y}|\bm{x}, \bm{\theta})}{{\tt P}(\bm{y} | \bm{x}, \mathcal{D})}\Big]\Big] \\
% =&\ \mathcal{ H}\big[{\tt P}(\bm{y} | \bm{x}, \mathcal{D})\big] - \mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(\bm{y} | \bm{x}, \bm{\theta})]\big]
% \end{split}
% \end{empheq}
% Strictly speaking, sequence-level mutual information requires the ensemble's predictive posterior to be combined as an \emph{expectation-of-products}, as it is assumed that the \emph{entire} sequence is generated using a \emph{particular} set of model parameters. We can also consider the expected pairwise KL-divergence (EPKL) between models in the ensemble as a measure of ensemble diversity:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{K}\big[\bm{y}, \bm{\theta} |  \bm{x}, \mathcal{D}\big] =&\ \mathbb{E}_{{\tt q}(\bm{\theta}){\tt q}(\bm{\tilde \theta})}\big[{\tt KL}[{\tt P}(\bm{y} | \bm{x}, \bm{\theta})\|{\tt P}(\bm{y} |\bm{x}, \bm{\tilde \theta})]\big] \\
% =&\ \mathbb{E}_{{\tt q}(\bm{\theta}){\tt q}(\bm{\tilde \theta})}\Big[\mathbb{E}_{{\tt P}(\bm{y}|\bm{x}, \bm{\theta})}\Big[\ln\frac{{\tt P}(\bm{y} | \bm{x}, \bm{\theta})}{{\tt P}(\bm{y} |\bm{x}, \bm{\tilde \theta})}\Big]\Big] \\
% =&\ \mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathbb{E}_{{\tt P}(\bm{y} | \bm{x}, \mathcal{D})}[\ln{\tt P}(\bm{y} | \bm{x}, \bm{\theta})] \big] - \mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(\bm{y} | \bm{x}, \bm{\theta})]\big] 
% \end{split}%\label{eqn:sequence-epkl-app}
% \end{empheq}
% This measure is an upper bound on the mutual information, obtainable via Jensen's inequality. The EPKL can be decomposed into an upper bound on the entropy of the predictive posterior and the expected entropy of each model. Thus, estimates of \emph{data uncertainty} are unchanged. The upper-bound on the estimates of \emph{total uncertainty} is the expected cross-entropy between each model and the predictive posterior. Another measure of ensemble diversity which can be considered is the mean KL-divergence between each model and the predictive posterior:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{M}\big[\bm{y}, \bm{\theta} |  \bm{x}, \mathcal{D}\big] =&\ \mathbb{E}_{{\tt q}(\bm{\theta})}\big[{\tt KL}[{\tt P}(\bm{y} | \bm{x}, \mathcal{D})\|{\tt P}(\bm{y}|\bm{x}, \bm{\theta})]\big] \\
% =&\  \mathbb{E}_{{\tt q}(\bm{\theta})} \Big[\mathbb{E}_{{\tt P}(\bm{y}|\bm{x}, \mathcal{D})}\Big[\ln\frac{{\tt P}(\bm{y} | \bm{x}, \mathcal{D})}{{\tt P}(\bm{y}|\bm{x}, \bm{\theta})}\Big]\Big] \\
% =&\ \mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathbb{E}_{{\tt P}(\bm{y} | \bm{x}, \mathcal{D})}[\ln{\tt P}(\bm{y} | \bm{x}, \bm{\theta})] \big] - \mathcal{ H}\big[{\tt P}(\bm{y} | \bm{x}, \mathcal{D})\big]
% %\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathbb{E}_{{\tt P}_{\tt EP}(\bm{y} | \bm{x}, \mathcal{D})}[\ln{\tt P}(\bm{y} | \bm{x}, \bm{\theta})] \big] - \mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(\bm{y} | \bm{x}, \bm{\theta})]\big]
% \end{split}%\label{eqn:sequence-epkl-app}
% \end{empheq}
% This is effectively the reverse-KL divergence counterpart to the sequence mutual information. This measure can be decomposed into the difference between of the expected cross entropy between each model and the predictive posterior and the entropy of the predictive posterior. We note that while mutual information and EPKL are defined strictly in terms of an \emph{expectation-of-products} predictive posterior, MKL can be defined relative to either an \emph{expectation-of-products} or a \emph{product-of-expectations}. This makes MKL the \emph{only} sequence-level measure of \emph{knowledge uncertainty} which only requires inference form the predictive posterior, rather than form \emph{each} model within the ensemble. Finally, it is trivial to show that the following relationship holds between mutual information, EPKL and MKL, conditional on the predictive posterior being an \emph{expectation of products}:
% \begin{empheq}{align}
% \begin{split}
% \mathcal{M}\big[\bm{y}, \bm{\theta} |  \bm{x}, \mathcal{D}\big]  =&\  \mathcal{K}\big[\bm{y}, \bm{\theta} |  \bm{x}, \mathcal{D}\big] - \mathcal{I}\big[\bm{y}, \bm{\theta} |  \bm{x}, \mathcal{D}\big]
% \end{split}%\label{eqn:sequence-epkl-app}
% \end{empheq}
% Thus, the bound between the mutual information and EPKL is MKL.

% \subsection{Derivation of Predictive Posterior}

% As discussed in section~\ref{sec:struct-uncertainty}, ensembles of auto-regressive models can be combined either as an \emph{expectation of products} or as a \emph{product of expectations}:
% \begin{empheq}{align}
% \begin{split}
% {\tt P}_{\tt EP}(\bm{y}| \bm{x}, \mathcal{D}) =&\ \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l}, \bm{x}, \bm{\theta}) \Big], \ {\tt P}_{\tt PE}(\bm{y}| \bm{x}, \mathcal{D}) =\ \prod_{l=1}^L \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(\bm{y} | \bm{y}_{<l}, \bm{x}, \bm{\theta})\Big]
% \end{split}%\label{eqn:ensemble-combinations}
% \end{empheq}
% Combining an ensemble as an expectation of products represents Bayesian model averaging at the \emph{sequence level} - it assumes that the whole sequence $\bm{y}$ is sampled from a single model. In contrast, a product of expectations represents Bayesian model averaging at the \emph{token level} - that only each individual $\bm{y}_l$ is drawn from a single model, and the tokens can be drawn from multiple models throughout the sequence. Combining the ensemble as a product of expectations is consistent with how an individual model is trained via teacher forcing - as a sequence of token-level predictions given a reference context. Furthermore, it is also consistent with how decisions are made within beam search - it is a sequence of \emph{token-level decisions}, where tokens chosen at every step in order to maximise the joint probability of the sequence generated so far. This explains why, on a conceptual level, a product-of-expectations combination yields superior BLEU and WER performance.

% Unfortunately, it is not possible (to our knowledge) to related the two combinations via an inequality. However, it is possible to shown that the upper bound on the negative log-likelihood in both cases is the mean token-level negative log-likelihood:
% \begin{empheq}{align}
% \begin{split}
% \ln{\tt P}_{\tt EP}(\bm{y}| \bm{x}, \mathcal{D}) =&\ \ln\mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l}, \bm{x}, \bm{\theta}) \Big] \geq \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\sum_{l=1}^L \ln{\tt P}(y_l | \bm{y}_{<l}, \bm{x}, \bm{\theta}) \Big]\\
% \ln{\tt P}_{\tt PE}(\bm{y}| \bm{x}, \mathcal{D}) =&\ \sum_{l=1}^L \ln \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(\bm{y} | \bm{y}_{<l}, \bm{x}, \bm{\theta})\Big] \geq \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\sum_{l=1}^L \ln{\tt P}(y_l | \bm{y}_{<l}, \bm{x}, \bm{\theta}) \Big]
% \end{split}%\label{eqn:ensemble-combinations}
% \end{empheq}
% This means that in the derivations below, the entropy of the predictive posterior obtained using either combination is larger the then expected entropy of each model.

% Note that in both of these approximations factorize out ${\tt P}(y_l | \bm{y}_{<l}^{(s)},  \bm{x}, \mathcal{D})$. How the obtain this depends on how the ensemble was combined. If the model is combined as a \emph{product of expectations}, the it is trivial to obtain the token-level predictive posterior:
% \begin{empheq}{align}
% \begin{split}
% {\tt P}(y_l | \bm{y}_{<l}^{(s)},  \bm{x}, \mathcal{D}) =&\  \mathbb{E}_{{\tt q}(\bm{\theta})}\big[{\tt P}(y_l | \bm{y}_{<l}^{(s)},  \bm{x}, \bm{\theta})\big]
% \approx\ \frac{1}{M}\sum_{m=1}^M{\tt P}(y_l | \bm{y}_{<l}^{(s)},  \bm{x}, \bm{\theta}^{(m)})
% \end{split}%\label{eqn:sequence-mi-app}
% \end{empheq}
% However, if the model is combined as an \emph{expectation of products}, then factorising the sequence-level posterior into the token-level posterior is more tricky:
% \begin{empheq}{align}
% \begin{split}
% {\tt P}(y_l | \bm{y}_{<l}^{(s)},  \bm{x}, \mathcal{D}) =&  \frac{{\tt P}(y_l,  \bm{y}_{<l}^{(s)},  \bm{x}, \mathcal{D})}{{\tt P}(\bm{y}_{<l}^{(s)},  \bm{x}, \mathcal{D})} = \frac{\mathbb{E}_{{\tt q}(\bm{\theta})}\big[{\tt P}(y_l,  \bm{y}_{<l}^{(s)},  \bm{x}, \bm{\theta})\big]}{\mathbb{E}_{{\tt q}(\bm{\theta})}\big[{\tt P}(\bm{y}_{<l}^{(s)},  \bm{x}, \bm{\theta})\big]}
% %\approx \frac{\frac{1}{M}\sum_{m}^M{\tt P}(y_l,  \bm{y}_{<l}^{(s)},  \bm{x}, \bm{\theta}^{(m)})}{\frac{1}{M}\sum_{m}^M{\tt P}(\bm{y}_{<l}^{(s)},  \bm{x}, \bm{\theta}^{(m)})}
% \end{split}%\label{eqn:sequence-mi-app}
% \end{empheq}
% where $\bm{y}_{<l}^{(s)}$ is a particular realization of the random variable $\bm{y}_{<l}$. The problem does not apply for the chain-rule decomposition for EPKL:

==> reviews.tex <==
TO Chair and Area Chair


Dear Chairs and Area Chairs,

We were disappointed with Reviewer 1s comments and concerned about R1 ability to appropriately assess the merits of our paper. We have provided a detailed reply to each of R1s points, and hope that it is clear that our concerns are not unfounded. 

Best Regards,
Authors. 


TO ALL REVIEWERS

Dear Reviewers,

Thank


Reviewer 2:





==> structured_uncertainty.tex <==
\section{Uncertainty for Structured Prediction}\label{sec:struct-uncertainty}

In this section the probabilistic framework for uncertainty estimation discussed in the previous section is applied to structured prediction. Consider auto-regressive models that map a $T$-length sequence of inputs $\{\bm{x}_1,\cdots,\bm{x}_T\} = \bm{X}$ to an $L$-length sequence of targets $\{y_1,\cdots,y_L\} = \bm{y}$:
\begin{empheq}{align}
{\tt P}(\bm{y}| \bm{X}, \bm{\theta}) =&\ \prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l},  \bm{X}; \bm{\theta})
\label{eqn:stuct-predict-autoreg}
\end{empheq}
In this model the distribution over each $y_l$ is conditioned on all the previous $\bm{y}_{<l} = \{y_1,\cdots,y_{l-1}\}$, which we shall refer to as the \emph{context}. This formulation describes all neural machine translation~\cite{bahdanau2015nmt, attentionisallyouneed}, end-to-end speech recognition \cite{las} and other related tasks. For these models uncertainty estimation can be examined at two levels - the \emph{token level}, which considers uncertainty in the prediction of a single $y_l$, and the \emph{sequence level}, which considers the uncertainty of predicting the entire sequence $\bm{y}$. 

Before we discuss uncertainty estimation, we first must consider how to obtain the predictive posterior from an ensemble of auto-regressive models. While there is only one way to express the predictive posterior ${\tt P}(y| \bm{x}, \mathcal{D})$ at the token-level, the sequence-level predictive posterior for auto-regressive models can be expressed either as an \emph{expectation-of-products} or a \emph{product-of-expectations}:
\begin{empheq}{align}
\begin{split}
{\tt P}_{\tt EP}(\bm{y}| \bm{X}, \mathcal{D}) =&\ \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l}, \bm{X}, \bm{\theta}) \Big], \ {\tt P}_{\tt PE}(\bm{y}| \bm{X}, \mathcal{D}) =\ \prod_{l=1}^L \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(y_l | \bm{y}_{<l}, \bm{X}, \bm{\theta})\Big]
\end{split}\label{eqn:ensemble-combinations}
\end{empheq}
Both are valid ways to do model combination\footnote{In the current Fairseq~\cite{fairseq} implementation ensembles are combined as a \emph{product-of-expectations}.}. However, the optimal ${\tt q}(\bm{\theta})$ will depend on the choice of combination approach. Consider the ${\tt q}(\bm{\theta})$ which maximizes the log-likelihood of a dataset $\mathcal{D} = \{\bm{y}^{(i)},\bm{X}^{(i)}\}_{i=1}^N$ under ${\tt P}(\bm{y}| \bm{X}, \mathcal{D})$ in the case of both decompositions:
% \begin{empheq}{align}
% \begin{split}
% {\tt \hat q}(\bm{\theta}) =&\ \arg\max_{{\tt q}(\bm{\theta})}\  \mathbb{E}_{\mathcal{D}}\Big[ \ln \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\prod_{l=1}^L {\tt P}(y_l | \bm{y}_{<l}, \bm{X}, \bm{\theta}) \Big]\Big] \\
% {\tt \tilde q}(\bm{\theta}) =&\ \arg\max_{{\tt q}(\bm{\theta})}\  \mathbb{E}_{\mathcal{D}}\Big[ \ln  \prod_{l=1}^L \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[{\tt P}(y_l | \bm{y}_{<l}, \bm{X}, \bm{\theta})\Big] \Big]
% \end{split}
% \end{empheq}
\begin{empheq}{align}
\begin{split}
{\tt \hat q}_{\tt EP}(\bm{\theta}) =&\ \arg\max_{{\tt q}(\bm{\theta})}\  \mathbb{E}_{\mathcal{D}}\Big[ \ln {\tt P}_{\tt EP}(\bm{y}| \bm{X}, \mathcal{D})\Big],\quad
{\tt \hat q}_{\tt PE}(\bm{\theta}) =\ \arg\max_{{\tt q}(\bm{\theta})}\  \mathbb{E}_{\mathcal{D}}\Big[ \ln  {\tt P}_{\tt PE}(\bm{y}| \bm{X}, \mathcal{D})\Big]
\end{split}
\end{empheq}
In the first case, ${\tt \hat q}_{\tt EP}(\bm{\theta})$ will maximize the \emph{joint} log-probability of all tokens in all sequences in the dataset $\mathcal{D}$, but not necessarily the \emph{conditional} log-probabilities of all tokens. In the latter case, ${\tt \hat q}_{\tt PE}(\bm{\theta})$ will maximize \emph{both} the \emph{joint} and \emph{conditional} probabilities of all tokens. Thus, ${\tt \hat q}_{\tt EP}(\bm{\theta})$ is not in general equal to  ${\tt \hat q}_{\tt PE}(\bm{\theta})$. This has two implications. Firstly, given a set of samples of parameters $\bm{\theta}^{(m)}$ from a particular ${\tt q}(\bm{\theta})$ and an inference method, it is not clear what is the best way to combine these models. Secondly, the choice of combination will affect uncertainty measures derived from ${\tt P}(\bm{y}| \bm{X}, \mathcal{D})$.
\todo{Make up my mind about EP vs PE in all approximations}

For auto-regressive models, the task of \emph{token-level} uncertainty estimation is isomorphic to uncertainty estimation in un-structured models as described in section~\ref{sec:ensembles}, given a known and fixed context $\bm{y}_{<l}$ \footnote{Further details are provided in appendix~\ref{apn:token-uncertainty}}. However, obtaining \emph{sequence-level} estimates of \emph{total}, \emph{data} and \emph{knowledge uncertainty} is both more challenging and interesting. Let's begin by stating that for sequence data we will work with length-normalized entropy and mutual information, called \emph{entropy rate} $\mathcal{\hat H}$ and \emph{mutual information rate} $\mathcal{\hat I}$, in order to be able to compare sequences of different lengths~\cite{information-theory}. Consider the mutual information rate between the model parameters $\bm{\theta}$ and the sequence $\bm{y}$:
\begin{empheq}{align}
\begin{split}
\underbrace{\mathcal{\hat I}\big[\bm{y}, \bm{\theta} |  \bm{X}, \mathcal{D}\big]}_{\text{Knowledge Uncertainty}} =&\ \underbrace{\mathcal{\hat H}\big[{\tt P}_{\tt EP}(\bm{y} | \bm{X}, \mathcal{D})\big]}_{\text{Total Uncertainty}} - \underbrace{\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{\hat H}[{\tt P}(\bm{y} | \bm{X}, \bm{\theta})]\big]}_{\text{Expected Data Uncertainty}}
\end{split}\label{eqn:sequence-mi}
\end{empheq}
This expression requires the evaluation of the entropy rate, which is defined as:
\begin{empheq}{align}
\begin{split}
\mathcal{\hat H}[{\tt P}(\bm{y} |  \bm{X}, \bm{\theta})] =&\ \frac{1}{L}\mathcal{H}[{\tt P}(\bm{y} |  \bm{X}, \bm{\theta})] = -\frac{1}{L}\sum_{\bm{y}\in\mathcal{Y}^L}{\tt P}(\bm{y} |  \bm{X}, \bm{\theta})\ln{\tt P}(\bm{y} |  \bm{X}, \bm{\theta})
\end{split}\label{eqn:sequence-entropy}
\end{empheq}
Unfortunately, this is intractable to evaluate due to the combinatorial explosion of the hypothesis space - there are a total of $|K|^L$ possible L-length sequences in $\mathcal{Y}^L$, where $K$ is the vocabulary size, and it is necessary to do a forward-pass through the network \emph{for each} hypothesis. Clearly, it is necessary to consider approximations to make this tractable. Furthermore, it is desirable that these approximations be consistent with high-performance inference techniques. In the following sections we examine two types of Monte-Carlo approximations for~\ref{eqn:sequence-entropy} and related uncertainty measures, which are identical in the limit, but have different attributes given a finite sample size.

\subsection{Chain-rule Monte-Carlo approximations}
Consider using the chain-rule of entropy~\cite{information-theory} to express~\ref{eqn:sequence-entropy} as a sum of expectations of conditional entropy. These expectations can then all be approximated via Monte-Carlo sampling as follows:
\begin{empheq}{align}
\begin{split}
\mathcal{\hat H}[{\tt P}(\bm{y} | \bm{X}, \bm{\theta})] =&\ \frac{1}{L}\sum_{l=1}^L \mathbb{E}_{{\tt P}(\bm{y}_{<l} | \bm{X}, \bm{\theta})}\big[\mathcal{H}[{\tt P}(y_l | \bm{X},\bm{y}_{<l}, \bm{\theta})]\big] \\
\approx&\ \frac{1}{SL}\sum_{l=1}^L\sum_{s=1}^S\mathcal{H}[{\tt P}(y_l | \bm{X},\bm{y}_{<l}^{(s)}, \bm{\theta})], \quad \forall\bm{y}_{<l}^{(s)} \subset \bm{y}^{(s)} \sim {\tt P}(\bm{y} | \bm{X}, \bm{\theta})
\end{split}\label{eqn:sum-approx}
\end{empheq}
Note that sequences sampled from ${\tt P}(\bm{y} | \bm{X}, \bm{\theta})$ can have different lengths, but we assume that all sequences are of length $L$ for notational convenience. Chain-rule based Monte-Carlo approximations can be obtained for mutual information rate:
\todo{Discussion of L needs to be earlier... Before 5...}
\begin{empheq}{align}
\begin{split}
\underbrace{\mathcal{\hat I}_{\text{MC}}^{(S)}\big[\bm{y}, \bm{\theta} |  \bm{X}, \mathcal{D}\big]}_{\text{Knowledge Uncertainty}}
\approx&\  \frac{1}{SL}\sum_{l,s}^{L,S}\mathcal{I}[y_l, \bm{\theta} | \bm{y}_{<l}^{(s)}, \bm{X}, \mathcal{D}],\quad  \forall\bm{y}_{<l}^{(s)} \subset \bm{y}^{(s)} \sim {\tt P}_{\tt EP}(\bm{y}| \bm{X}, \mathcal{D}) %\\
%\approx&\ \underbrace{\frac{1}{SL}\sum_{l,s}^{L,S}\mathcal{H}\big[{\tt P}(y_l | \bm{y}_{<l}^{(s)}, \bm{X}, \mathcal{D})\big]}_{\text{Total Uncertainty (TU)}} - \underbrace{\frac{1}{SL}\sum_{l,s}^{L,S}\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(y_l | \bm{y}_{<l}^{(s)}, \bm{X}, \bm{\theta})]\big]}_{\text{Expected Data Uncertainty (DU)}} %\\
%\mathcal{\hat I}_{\text{BS}}^{(S)}\big[\bm{y}, \bm{\theta} |  \bm{X}, \mathcal{D}\big] \approx&\  \frac{1}{L}\sum_{l,s}^{L,S}\pi_s\mathcal{I}[y_l, \bm{\theta} | \bm{y}_{<l}^{(s)}, \bm{X}, \mathcal{D}],\ \bm{y}^{(s)} \in \mathcal{B},\  \pi_s =\frac{{\tt P}_{\tt EP}(\bm{y}^{(s)}| \bm{X}, \mathcal{D})}{\sum_{s'} {\tt P}_{\tt EP}(\bm{y}^{(s')}| \bm{X}, \mathcal{D})}
\end{split}\label{eqn:sequence-mi-chain}
\end{empheq}
A similar approximation for sequence expected pairwise KL-divergence (EPKL) $\mathcal{\hat K}^{(S)}\big[\bm{y}, \bm{\theta} |  \bm{X}, \mathcal{D}]$ is described in appendix~\ref{apn:derivations}. Given a set of consistent contexts $\bm{y}_{<l} \subset \bm{y}\ \forall l< L$, these approximations essentially are averages of token-level uncertainty estimates. The quality of these approximations depends on several factors. Firstly, from which predictive distribution are the hypotheses drawn. While all these measures are defined in terms of sampling from an \emph{expectation-of-products} posterior, samples can also be drawn from a \emph{product-of-expectations}. The choice boils down to which distributions yields higher-quality samples given an inference procedure. Secondly, quality depends the number of samples drawn and the bias of the inference scheme. Finally, inference is typically done via beam-search, where each unique hypothesis is seen exactly once. Thus, the uncertainty of each hypothesis $\bm{y}^{(s)}$ within a beam $\mathcal{B}$ should be weighted in proportion to it's probability ${\tt P}(\bm{y}^{(s)}| \bm{X}, \mathcal{D})$:
\todo{Beam search discussion is a horror. Before (11) - really using Beam to get a "good" set of hypotheses from a vast space - sampling will need a large number of samples given the dimensionalities}
\begin{empheq}{align}
\begin{split}
\underbrace{\mathcal{\hat I}_{\text{BS}}^{(S)}\big[\bm{y}, \bm{\theta} |  \bm{X}, \mathcal{D}\big]}_{\text{Knowledge Uncertainty}} \approx&\  \frac{1}{L}\sum_{l,s}^{L,S}\pi_s\mathcal{I}[y_l, \bm{\theta} | \bm{y}_{<l}^{(s)}, \bm{X}, \mathcal{D}],\ \bm{y}^{(s)} \in \mathcal{B},\  \pi_s =\frac{{\tt P}(\bm{y}^{(s)}| \bm{X}, \mathcal{D})}{\sum_{s'} {\tt P}(\bm{y}^{(s')}| \bm{X}, \mathcal{D})} \\
\approx&\ \underbrace{\frac{1}{L}\sum_{l,s}^{L,S}\pi_s\mathcal{H}\big[{\tt P}(y_l | \bm{y}_{<l}^{(s)}, \bm{X}, \mathcal{D})\big]}_{\text{Total Uncertainty (TU)}} - \underbrace{\frac{1}{L}\sum_{l,s}^{L,S}\pi_s\mathbb{E}_{{\tt q}(\bm{\theta})}\big[\mathcal{H}[{\tt P}(y_l | \bm{y}_{<l}^{(s)}, \bm{X}, \bm{\theta})]\big]}_{\text{Expected Data Uncertainty (DU)}}
\end{split}\label{eqn:sequence-mi-chain-bs}
\end{empheq}


\subsection{Joint Sequence-level Monte-Carlo approximations}
An alternative Monte-Carlo approximation to~\ref{eqn:sequence-entropy} based on the joint distribution is the following:
\begin{empheq}{align}
\begin{split}
\mathcal{\hat H}^{(S)}\big[{\tt P}(\bm{y}|  \bm{X}, \bm{\theta})\big] \approx&\ -\frac{1}{SL}\sum_{s=1}^S \ln {\tt P}(\bm{y}| \bm{X},  \bm{\theta}),\ \bm{y}^{(s)} \sim {\tt P}(\bm{y}|  \bm{X}, \bm{\theta})
\end{split}\label{eqn:mc-sequence-entropy}
\end{empheq}
While the approximations~\ref{eqn:sum-approx} and~\ref{eqn:mc-sequence-entropy} yield the same result in the limit as $S\rightarrow\infty$, ~\ref{eqn:mc-sequence-entropy} only considers $L$ terms for each sample $\bm{y}^{(s)}$, and therefore converges slower than ~\ref{eqn:sum-approx}, which considers $KL$ terms per sample. Thus, for a finite $S$ approximation~\ref{eqn:mc-sequence-entropy} may yield poorer uncertainty estimates associated with an input $\bm{X}$. However, single-sample uncertainty estimates derived from~\ref{eqn:mc-mean-kl} are more sensitive to the uncertainty \emph{in a particular hypothesis}, and may therefore be better suited for error detection. This is similar to considering the log-likelihood of the max-class in unstructured prediction~\cite{malinin-thesis}. An approximation based on~\ref{eqn:mc-sequence-entropy} can be obtained for the mutual information rate:
\todo{Be more clear? Bad description of that arc stuff. probability of distribution vs sample. Mutual info via joint samples. Subtleties on sample draws. }
\begin{empheq}{align}
\begin{split}
\mathcal{\hat I}^{(S)}\big[\bm{y}, \bm{\theta} |  \bm{X}, \mathcal{D}\big] \approx&\  \frac{1}{SL}\sum_{s=1}^S\ln \frac{{\tt P}(\bm{y}^{(s)}| \bm{X},  \bm{\theta}^{(s)})}{{\tt P}_{\tt EP}(\bm{y}^{(s)}| \bm{X},  \mathcal{D})},\ \bm{y}^{(s)} \sim {\tt P}(\bm{y}| \bm{X},  \bm{\theta}^{(s)}), \bm{\theta}^{(s)} \sim {\tt q}(\bm{\theta})
\end{split}\label{eqn:mc-mutual-information}
\end{empheq}
This can be trivially expanded to yield Monte-Carlo estimates of \emph{total} and \emph{data uncertainty}. However, this approximation requires sampling from \emph{each} model in the ensemble, and evaluating the joint probability of the hypothesis using the predictive posterior, which is computationally expensive. Instead, we consider the following approximation:
\begin{empheq}{align}
\begin{split}
\underbrace{\mathcal{\hat M}_{\text{MC}}^{(S)}\big[\bm{y}, \bm{\theta} |  \bm{X}, \mathcal{D}\big]}_{\text{Knowledge Uncertainty}} \approx&\  \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\frac{1}{SL}\sum_{s=1}^S\ln \frac{{\tt P}(\bm{y}^{(s)} | \bm{X}, \mathcal{D})}{{\tt P}(\bm{y}^{(s)} | \bm{X},  \bm{\theta})}\Big],\ \bm{y}^{(s)} \sim {\tt P}(\bm{y}| \bm{X}, \mathcal{D}) %\\
%=&\  \underbrace{\frac{1}{SL}\sum_{s=1}^S\mathbb{E}_{{\tt q}(\bm{\theta})}\big[-\ln{\tt P}(\bm{y}^{(s)}| \bm{X},  \bm{\theta})\big]}_{\text{Expected Data Uncertainty (eSCR)}} - \underbrace{\frac{1}{SL}\sum_{s=1}^S -\ln{\tt P}(\bm{y}^{(s)}| \bm{X}, \mathcal{D})}_{\text{Total Uncertainty (SCR)}}
\end{split}\label{eqn:mc-mean-kl}
\end{empheq}
This yields the mean KL-divergence rate (MKL) between each model and the predictive posterior. This is a measure of ensemble diversity and, therefore, \emph{knowledge uncertainty}. MKL doesn't require sampling from each individual model, and can be evaluated using samples from either ${\tt P}_{\tt EP}(\bm{y}| \bm{X}, \mathcal{D})$ or ${\tt P}_{\tt EP}(\bm{y}| \bm{X}, \mathcal{D})$. If inference is done via beam-search, the MKL of each hypothesis should be weighted in proportion to it's probability:
\begin{empheq}{align}
\begin{split}
\mathcal{\hat M}_{\text{BS}}^{(S)}\big[\bm{y}, \bm{\theta} |  \bm{X}, \mathcal{D}\big] \approx&\  \mathbb{E}_{{\tt q}(\bm{\theta})}\Big[\sum_{s=1}^S \frac{ \pi_s}{L} \ln \frac{{\tt P}(\bm{y}^{(s)} | \bm{X}, \mathcal{D})}{{\tt P}(\bm{y}^{(s)} | \bm{X},  \bm{\theta})}\Big],   \bm{y}^{(s)} \in \mathcal{B},  \pi_s =\frac{{\tt P}(\bm{y}^{(s)}| \bm{X}, \mathcal{D})}{\sum_{s'} {\tt P}(\bm{y}^{(s')}| \bm{X}, \mathcal{D})} \\
=&\  \underbrace{\sum_{s=1}^S\frac{ \pi_s}{L}\mathbb{E}_{{\tt q}(\bm{\theta})}\big[-\ln{\tt P}(\bm{y}^{(s)}| \bm{X},  \bm{\theta})\big]}_{\text{Expected Data Uncertainty (eSCR)}} - \underbrace{\sum_{s=1}^S \frac{\pi_s}{L}\big[-\ln{\tt P}(\bm{y}^{(s)}| \bm{X}, \mathcal{D})\big]}_{\text{Total Uncertainty (SCR)}}
\end{split}\label{eqn:mc-mean-kl-bs}
\end{empheq}
MKL decomposes into entropy of the predictive posterior (SCR), a measure of \emph{total uncertainty}, and the mean cross-entropy between each model and predictive posterior (eSCR), a measure of \emph{data uncertainty}. Properties of these approximation are further discussed in appendix~\ref{apn:derivations}.
%7) “ … at odds with standard inference procedures which yield biased samples from each model” - what exactly are you referring to, reference?









